Counterfactual Action Evaluation, Observation Bottlenecks, and Representation Geometry in Joint-Embedding Predictive World Models

Low latent prediction error does not establish that a world model distinguishes the consequences of its actions. We introduce an evaluation protocol that traces the same intervention through simulator state, raster observations, target embeddings, and predictor outputs. Exact simulator-state forks in a controlled deformable-physics testbed reveal distinct bottlenecks. Changed commands alter particle motion, yet 41.5% of one-step raster pairs are identical. Observation loss is not the whole explanation: among 579 high-visibility counterfactuals, median predictor-to-target response is 0.0051 and 0.0217 across two seeds, falling to 0.0027 and 0.0116 after variance normalization. An isotropic state perturbation matched to the target counterfactual embedding shift produces 190x and 53x larger predictor changes on the same visible pairs, isolating action-path under-use rather than a dead or globally shrunk predictor. MSE-only training gives 8.36x lower 10-step latent error in matched seeds, but in spectrally concentrated spaces; one VICReg target encoder is also strongly concentrated, so neither error nor rank alone certifies physical state. Finally, stiffness remains near chance even from full-resolution rasters and mechanical state while privileged material parameters decode perfectly, indicating weak identifiability under this excitation rather than encoder discard. These results motivate auditing physical effect, observation visibility, representation geometry, and action dependence separately.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}
\begin{enumerate}
\setlength{\itemsep}{1pt}
\setlength{\parsep}{0pt}
\Needspace{6\baselineskip}
\item {\bf Claims}
\item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\item[] Answer: \answerYes{}
\item[] Justification: The abstract and Sections 1--5 separate physical, observation, representation, and predictor-side evidence and scope each claim to the tested simulator/checkpoints.

\Needspace{6\baselineskip}
\item {\bf Limitations}
\item[] Question: Does the paper discuss the limitations of the work performed by the authors?
\item[] Answer: \answerYes{}
\item[] Justification: Section~\ref{sec:limitations} and the appendices discuss observation quantization, actuator assumptions, validation reuse, replay differences, seed counts, and probe limitations.

\Needspace{6\baselineskip}
\item {\bf Theory assumptions and proofs}
\item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
\item[] Answer: \answerNA{}
\item[] Justification: The paper makes no theorem or proof claims. Equations define the implemented model, simulator, and metrics.

\Needspace{6\baselineskip}
\item {\bf Experimental result reproducibility}
\item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
\item[] Answer: \answerYes{}
\item[] Justification: Appendices~\ref{app:repro}--\ref{app:provenance} specify source hashes, model configurations, the validation-only evaluator, exact local replay diff, split policy, and the earlier Linux-replay distinction.

\Needspace{6\baselineskip}
\item {\bf Open access to data and code}
\item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
\item[] Answer: \answerYes{}
\item[] Justification: The anonymous OSF artifact linked in Appendix~\ref{app:repro} provides the canonical observation tensor, all ten final checkpoints, source code, cached metrics, manifests, and reproduction instructions required to rerun the reported checkpoint evaluation without retraining.

\Needspace{6\baselineskip}
\item {\bf Experimental setting/details}
\item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
\item[] Answer: \answerYes{}
\item[] Justification: Section~\ref{sec:setup}, Section~\ref{sec:protocol}, and the appendices state data splits, objectives, optimization, preprocessing, probe settings, and checkpoint selection.

\Needspace{6\baselineskip}
\item {\bf Experiment statistical significance}
\item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
\item[] Answer: \answerYes{}
\item[] Justification: Section~\ref{sec:protocol} distinguishes episode-bootstrap confidence intervals from descriptive interquartile bands. Two-seed objective results display both seeds directly and make no significance or equivalence claim.

\Needspace{6\baselineskip}
\item {\bf Experiments compute resources}
\item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
\item[] Answer: \answerYes{}
\item[] Justification: Appendix~\ref{app:repro} reports the MPS training system, 8 GiB memory, logged run times, CPU evaluation threads, and separately recorded execution environments.

\Needspace{6\baselineskip}
\item {\bf Code of ethics}
\item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
\item[] Answer: \answerYes{}
\item[] Justification: The work concerns synthetic simulator data and does not involve private data, human participants, or deployment decisions.

\Needspace{6\baselineskip}
\item {\bf Broader impacts}
\item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
\item[] Answer: \answerYes{}
\item[] Justification: The final appendix discusses more reliable evaluation as a benefit and overgeneralization of the controlled findings as a risk.

\Needspace{6\baselineskip}
\item {\bf Safeguards}
\item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
\item[] Answer: \answerNA{}
\item[] Justification: The study does not introduce a high-risk generative or decision-making asset.

\Needspace{6\baselineskip}
\item {\bf Licenses for existing assets}
\item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
\item[] Answer: \answerYes{}
\item[] Justification: Original project code in the anonymous artifact is released under MIT; the adapted MLS-MPM implementation retains the upstream MIT notice associated with Hu et al. (2018). The artifact documents provenance and required notices in \texttt{THIRD\_PARTY\_LICENSES.md} and \texttt{LICENSE\_AUDIT.md}; no external dataset or pretrained model is used.

\Needspace{6\baselineskip}
\item {\bf New assets}
\item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
\item[] Answer: \answerYes{}
\item[] Justification: The included README, source audit, configurations, provenance hashes, Phase-2 CSVs, and generation scripts document the evaluation assets and distinguish the original dump from the earlier cross-platform replay.

\Needspace{6\baselineskip}
\item {\bf Crowdsourcing and research with human subjects}
\item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)?
\item[] Answer: \answerNA{}
\item[] Justification: The study does not involve crowdsourcing or human subjects.

\Needspace{11\baselineskip}
\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
\item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
\item[] Answer: \answerNA{}
\item[] Justification: The study does not involve human subjects; IRB review is not applicable.

\Needspace{6\baselineskip}
\item {\bf Declaration of LLM usage}
\item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
\item[] Answer: \answerNA{}
\item[] Justification: No LLM is a component of the predictive model, simulator, or evaluated probe methods.

\end{enumerate}


==> data/reviewer_strengthening/01_simulator_counterfactual/table_simulator_counterfactual.tex <==
% Candidate table. Not manuscript prose. Values from aggregate_metrics.json.

\begin{tabular}{lrrr}
\toprule
Intervention (h=1) & median RMS pos $\Delta$ & identical uint8 frac. & median $v$ RMS $\Delta$ \\
\midrule
shuffled-same-time & 1.1906e-05 & 0.4153 & 0.002386 \\
neutral            & 7.8767e-06 & 0.5793 & 0.001577 \\
force-reversed (OOD) & 1.5762e-05 & 0.5203 & 0.003156 \\
\bottomrule
\end{tabular}

\begin{tabular}{lrrrr}
\toprule
Checkpoint & pred MSE (shuf) & tgt MSE (shuf) & median capture & excluded $N$ \\
\midrule
vicreg nocrop s42 last.pt & 1.9272e-06 & 1.8069e-06 & 0.01647 & 1273/3000 \\
vicreg nocrop s43 last.pt & 2.5879e-06 & 3.1272e-06 & 0.06699 & 1256/3000 \\
\bottomrule
\end{tabular}


==> data/reviewer_strengthening/02_action_distance/table_action_distance.tex <==
% Action-distance quintiles on normalized L2, defined before inspecting predictor trends.

\begin{tabular}{lrrrr}
\toprule
Quintile & n & action L2 med. & phys RMS pos med. & pred MSE s42 med. \\
\midrule
1 (smallest swap) & 600 & 1.475 & 6.75e-06 & 6.02e-07 \\
3 & 600 & 2.589 & 1.24e-05 & 2.12e-06 \\
5 (largest swap) & 600 & 3.794 & 1.85e-05 & 5.17e-06 \\
\bottomrule
\end{tabular}


==> tables/observability_rows.tex <==
EMA, single frame & Linear & 14 & 32.0--35.0 & 100.0--100.0 \\
EMA, single frame & MLP & 14 & 30.0--39.0 & 100.0--100.0 \\
EMA, history & Linear & 8 & 31.5--36.5 & 100.0--100.0 \\
EMA, history & MLP & 8 & 30.5--37.5 & 100.0--100.0 \\
Raster, single frame & Linear & 7 & 33.5--33.5 & 100.0--100.0 \\
Raster, single frame & MLP & 7 & 33.5--33.5 & 100.0--100.0 \\
Raster, history & Linear & 1 & 33.5--33.5 & 100.0--100.0 \\
Raster, history & MLP & 1 & 33.0--33.0 & 50.5--50.5 \\


==> tables/per_seed_rows.tex <==
VICReg + action & 42 & 0.07551 & 0.61990 & 1.21104 & 4.447 & 12.27 & 0.178 \\
VICReg + action & 43 & 0.06968 & 0.61641 & 1.10064 & 7.152 & 5.78 & 0.333 \\
VICReg, no action & 42 & 0.07474 & 0.59500 & 1.14593 & 4.282 & 11.67 & 0.182 \\
VICReg, no action & 43 & 0.09871 & 0.71149 & 1.27055 & 4.466 & 13.44 & 0.184 \\
VICReg + action & 44 & 0.07080 & 0.50848 & 1.06394 & 4.820 & 13.06 & 0.174 \\
VICReg, no action & 44 & 0.07525 & 0.54499 & 1.06228 & 4.317 & 12.24 & 0.149 \\
VICReg + action & 45 & 0.08055 & 0.55217 & 1.08827 & 3.703 & 13.14 & 0.184 \\
VICReg, no action & 45 & 0.07421 & 0.55050 & 1.16764 & 3.724 & 12.70 & 0.157 \\
MSE-only + action & 42 & 0.00707 & 0.07421 & 0.14783 & 0.713 & 4.31 & 0.453 \\
MSE-only + action & 43 & 0.00549 & 0.06330 & 0.12866 & 0.518 & 3.46 & 0.512 \\


==> tables/per_seed_rows_phase2.tex <==
VICReg + action & 42 & 0.07551 & 0.61990 & 1.21103 & 4.447 & 5.97 & 4.64 \\
VICReg + action & 43 & 0.06968 & 0.61641 & 1.10064 & 7.152 & 2.44 & 2.11 \\
VICReg, no action & 42 & 0.07474 & 0.59499 & 1.14593 & 4.282 & 6.16 & 4.98 \\
VICReg, no action & 43 & 0.09871 & 0.71149 & 1.27055 & 4.466 & 6.54 & 5.48 \\
VICReg + action & 44 & 0.07080 & 0.50848 & 1.06394 & 4.820 & 9.24 & 7.94 \\
VICReg, no action & 44 & 0.07525 & 0.54499 & 1.06228 & 4.317 & 6.93 & 5.81 \\
VICReg + action & 45 & 0.08055 & 0.55217 & 1.08827 & 3.703 & 6.25 & 5.12 \\
VICReg, no action & 45 & 0.07421 & 0.55050 & 1.16764 & 3.724 & 8.27 & 6.82 \\
MSE-only + action & 42 & 0.00707 & 0.07421 & 0.14783 & 0.713 & 4.30 & 4.50 \\
MSE-only + action & 43 & 0.00549 & 0.06330 & 0.12866 & 0.518 & 3.59 & 3.69 \\


==> tables/phase2_counterfactual_rows.tex <==
42 & 579 & 4.13e-04 & 2.14e-06 & 0.0051 & 0.0027 & 59.5 & 189.5 \\
43 & 579 & 1.35e-04 & 3.04e-06 & 0.0217 & 0.0116 & 16.9 & 53.2 \\


==> tables/probe_rows.tex <==
VICReg + a & 42 & 99.90 & 30.05 & 39.70 & +0.017 \\
VICReg + a & 43 & 100.00 & 30.30 & 39.60 & +0.011 \\
VICReg, no a & 42 & 100.00 & 30.05 & 38.60 & +0.000 \\
VICReg, no a & 43 & 100.00 & 35.35 & 40.70 & +0.000 \\
VICReg + a & 44 & 100.00 & 31.10 & 39.70 & +0.039 \\
VICReg, no a & 44 & 100.00 & 33.10 & 43.40 & +0.000 \\
VICReg + a & 45 & 99.75 & 32.65 & 38.35 & -0.010 \\
VICReg, no a & 45 & 99.15 & 30.90 & 41.65 & +0.000 \\
MSE + a & 42 & 100.00 & 33.25 & 39.50 & +0.018 \\
MSE + a & 43 & 100.00 & 34.85 & 36.00 & +0.002 \\


==> tables/rank_horizon_rows.tex <==
VICReg+a & 42 & 5.97 & 4.64 & 8.26 & 4.66 & 9.38 & 4.61 & 9.91 & 4.64 \\
VICReg+a & 43 & 2.44 & 2.11 & 3.19 & 2.14 & 3.70 & 2.13 & 4.49 & 2.10 \\
VICReg-noa & 42 & 6.16 & 4.98 & 8.00 & 4.99 & 8.97 & 5.01 & 8.11 & 4.94 \\
VICReg-noa & 43 & 6.54 & 5.48 & 8.91 & 5.43 & 10.94 & 5.36 & 11.17 & 5.37 \\
VICReg+a & 44 & 9.24 & 7.94 & 10.44 & 7.96 & 10.87 & 7.95 & 10.08 & 7.93 \\
VICReg-noa & 44 & 6.93 & 5.81 & 8.86 & 5.81 & 9.95 & 5.75 & 8.98 & 5.73 \\
VICReg+a & 45 & 6.25 & 5.12 & 8.45 & 5.15 & 10.07 & 5.15 & 10.85 & 5.13 \\
VICReg-noa & 45 & 8.27 & 6.82 & 9.93 & 6.91 & 10.38 & 6.80 & 9.20 & 6.73 \\
MSE+a & 42 & 4.30 & 4.50 & 4.08 & 4.56 & 3.89 & 4.53 & 3.54 & 4.42 \\
MSE+a & 43 & 3.59 & 3.69 & 3.38 & 3.71 & 3.21 & 3.71 & 2.94 & 3.67 \\


==> tables/secondary_rows.tex <==
Shuffled & 3000 & 1.191 & 2.386 & 41.53 \\
Mean action & 3000 & 0.788 & 1.577 & 57.93 \\
Force reversed & 3000 & 1.576 & 3.156 & 52.03 \\
Force rotated & 3000 & 1.111 & 2.232 & 54.57 \\
Force scaled & 3000 & 0.394 & 0.789 & 40.40 \\
Contact shifted & 3000 & 0.464 & 0.903 & 47.33 \\


==> tables/stiffness_positive_rows.tex <==
Mechanical $x,v,C,F$ & 28.5--39.5 & 100.0--100.0 \\
Mechanical history & 33.0--33.5 & 100.0--100.0 \\
Float $64\times64$ raster & 33.0--33.5 & 100.0--100.0 \\
Float raster history & 33.0--33.5 & 50.5--100.0 \\
uint8 $64\times64$ raster & 32.5--34.0 & 100.0--100.0 \\
uint8 raster history & 33.5--33.5 & 50.5--100.0 \\
Privileged $\mu,\lambda$ (linear) & 66.5 & 49.5 \\
Privileged $\mu,\lambda$ (MLP) & 100.0 & 50.0 \\

